Designing for Participation and Change in Digital Institutions

Whether we recognize it or not, the Internet is rife with exciting and original institutional forms that are transforming social organization on and offline. Issues of governance in these Internet platforms and other digital institutions have posed a challenge for software engineers, many of whom have little exposure to the relevant history or theory of institutional design. Here, we offer one useful framework with an aim to stimulate dialogue between computer scientists and political scientists. The dominant guiding practices for the design of digital institutions to date in human-computer interaction, computer-supported cooperative work, and the tech industry at large have been an incentive-focused behavioral engineering paradigm, a collection of atheoretical approaches such as A/B-testing, and incremental issue-driven software engineering. One institutional analysis framework that has been useful in the design of traditional institutions is the body of resource governance literature known as the "Ostrom Workshop". A key finding of this literature that has yet to be broadly incorporated in the design of many digital institutions is the importance of including participatory change process mechanisms in what is called a "constitutional layer" of institutional design---in other words, defining rules that allow and facilitate diverse stakeholder participation in the ongoing process of institutional design change. We explore to what extent this consideration is met or could be better met in three varied cases of digital institutions: cryptocurrencies, cannabis informatics, and amateur Minecraft server governance. Examining such highly varied cases allows us to demonstrate the broad relevance of constitutional layers in many different types of digital institutions.

==> bikerack.tex <==

%The dominant image of digital institution design is from the image of a venture capital-funded technologist-turned-entrepreneur: Bill Gates's Microsoft extending its operating system into web browsers, Mark Zuckerberg's Facebook newsfeed algorithmically filtering your friends' content, or Travis Kalanick's Uber reconfiguring urban mobility. But this prevailing popular image of top-down, elite-driven institutional design is incomplete. Falling technology costs, increased connectivity, and ever more pervasive information technologies have contributed to an explosion of amateurs designing and leading large and influential online communities. Centrally-hosted services like Facebook, Twitter, Reddit, World of Warcraft, and Coursera are all providers of turnkey community creation tools that make it easy to organize large collectives. More personal self-hosted services like Apache, phpBB, MediaWiki, and even Minecraft let people build highly-customizable platforms of their own, and host small communities on their own terms. Amateurs and volunteers thus play crucial roles developing new digital institutions alongside elite-driven strategies. What unites these top-down and bottom-up patterns of digital institution design is a reliance on intuitions, folk theories, and iteration rather than consciously designing new institutions by translating successful strategies, incentives, and structures from other successful institutions.


%Their efforts fulfill the promise of the Internet as a decentralized medium of personal and community empowerment. The challenges these digital institution builders face are not new: the biggest challenges facing humanity---climate change, over-fishing, antibiotic resistance, deforestation, and overpopulation---are all commons dilemmas characterized by the benefits of non-cooperation accruing to individuals, the costs accruing to others, and the aggregate harms exceeding the benefits. The tragedy of the commons is an incredibly intransigent problem, and it is baked into the challenge of starting an online community, as increasing numbers of users place increasing demands on server resources, network bandwidth, and support staff.
%

% \pk{Add citations}  
%The result is a sea of quiet failures out of which inexplicable successes occasionally rise. 
%

%Policymakers and bureaucrats struggle to align their interpretations and regulations with rapidly-changing technological capacities and social practices. Social scientists and humanists also wade into this sea of quiet failures with well-intentioned but unsustainable one-off prototypes, \textit{post-hoc} enumerations of ``predictable'' failures, and deterministic admonitions about the hubris of engineering social systems. 

%As the once rare and privileged opportunity to design a digital institution reaches more people, and transforms passive users to active organizers, there is a growing appreciation that understanding how society \textit{does} work tells us almost nothing about how society \textit{could} work. With its track record of design innovation, of integrating social theories into digital contexts, and of embracing a mixture of qualitative and quantitative approaches to sociotechnical assemblies, the HCI community is strategically positioned to  bring users, designers, engineers, social scientists, and artists together to more fully explore the  space of possible digital institutions. 


%The tragedy of the commons is an incredibly intransigent problem, and it is baked into the challenge of starting an online community, as increasing numbers of users place increasing demands on server resources, network bandwidth, support staff, and other shared resources.
 
 %Brian's intro: Lots of examples of institutional failures in digital systems recently, this is not a new problem and smart people have identified sustainable solutions, one of hte most influential of these  is called the Ostrom framework. Let's look at how the Ostrom framework could be applied to three wildly different examples

%the micro is always situated in the macro?

%When we think of digital institution design beyond academic prototypes, the major actors seem to be large institutions: social media companies like Facebook and Twitter and important peer-produced institutions like Stack Exchange and Reddit, all engineered more and less centrally by engineers, and then used by users under the constraints established by the code.  There are exceptions.  Wikipedia includes users in its central policy apparatus, allows policy differences between the different language encyclopedias, and enjoys a large community of sovereign satellite institutions via self-hosted MediaWiki installations.  Such self-hosted or otherwise sovereign exceptions continue to play only a peripheral role in our understanding of the importance of digital institution design. But they are one of the most promising settings for empirically researching the effects of digital institution design while also serving as a critical counter-factual about the possibility of alternative political economies among digital institutions.



%We require a framework that can make sense of players of massively multiplayer online games (MMOGs) authoring client hacks to implement gaming guild hierarchies, users empowering themselves to establish and govern Reddit sub-communities, support groups building peer communities around online forums, and friends sharing web servers.


%All of these challenges are amplified in the case of popular amateur-hosted self-governing online multiplayer game servers like Counterstrike and Minecraft, whose users are young, and whose closest antecedents in political philosophy are the survivors from {\it The Lord of the Flies}, whose brief reign over a castaway island ended famously in murder and anarchy. Here we discuss the governance styles of sovereign server administrators of the virtual world game Minecraft.

% the design, implementation, and evaluation of comparatively small-scale socio-technical assemblies of individuals, groups, or organizations rather than digital institutions occurring at the level of an entire market or society. To be fair, the opportunities to design digital institutions were rare and privileged for years, but the pervasiveness and consequences of contemporary digital institutions suggest these re-appraising scarcity assumptions and engaging with the accelerating opportunities to design digital institutions.

%To accomplish our aim, CHI and CSCW must take on topics of sociology, economics, policy, and politics in addition to our foundational grounding in social and cognitive psychology.
%social scientists and humanists to play an earlier role---in the development process of digital systems: in the design of digital institutions.  

%Coming from an ecological tradition, Ostrom's methods already integrate the best of economics, sociology, psychology, and ecosystem science, and are a natural candidate for integration with HCI's similarly diverse canon.

%\subsection{The Ostrom Workshop and the resource management perspective}.

%Off of these main contributions, four branches of scholarship have leveraged the Ostromite resource management perspective to advance insight into digital institutions.  These literatures are on the knowledge commons, the effectiveness of bottom-up norms, the policy analyses of digital spaces, and the prescriptive design of digital institutions.
%\subsubsection{Knowledge commons}

%In collaboration with Charlotte Hess, she applies the resource management perspective to Information Age problems of peer production, digital coordination, and precursors to open science \cite{Hess:2007we}.

%\subsubsection{Norm emergence, functioning, and design}

%Many digital institutions seem to function successfully only because of emergent normed behaviors that were neither designed into the system nor anticipated by its designers, and many investigations of such systems have relied on the  Ostrom Workshop's frameworks for describing norm systems. 

%\subsubsection{Digital policy analysis}

%\subsubsection{Prescriptive approach to digital institution design}

%Kraut and Resnick, while coming mostly from the perspectives of social psychology and information science, draw on Ostrom's 

%labs of computer scientists Jeremy Pitt and Ada Diaconescu, whose work in the 

%uses the Ostrom Workshop's framework 
% \sf{\pk{Summarize our contributions on top of this literature}We build upon these efforts by distilling   key components of several more unexplored resource management theories into a framework for integrating technological, economic, cultural, and political perspectives on institutions, for use by digital institution designers.}

% \subsection{Alternative frameworks}
% \brian{Candidate section to cut}

% Beyond the Ostrom Workshop, there are many alternative frameworks for reasoning about institutional analysis and design:
% \begin{description}
% \item[Organizational theory.] Organization theory takes a goal oriented approach to the multitudinous ways to structure organizations. Where resource management treats agents as having sundry goals, org theory is appropriate for systems whose agents are subservient to a single goal.  Several pieces of work in the HCI and CSCW communities have leveraged organizational theory for practical analysis and design, including work on collective action among Reddit moderators against its management~\cite{Matias:2016db}, large comparative analyses of for-profit Wikia wikis~\cite{Shaw:2014gv}, the transmission of writing conventions in the process of authoring collaborative written works~\cite{Rotabi:2017cg}, and several others~\cite{Hill:2017tx}.
% \item[Network science.] Many researchers have used networks to measure collective action outcomes in digital institutions at the scale of the team \cite{krafft2012topic,Huang:2013gb,Chung:2014dc,Muller:2015vz,Muller:2015ut} and higher \cite{Szell:2010jb,Ugander:2012vx}. A major advantage of the network approach is that it is amenable to lab experiments in addition to  observational studies---a medium researchers have uses to test the effects of different  information transmission structures  on collective performance \cite{Mason:2012dl,Mason:2008vd,Kearns:2006wj}.
% \item[Social psychology.] Social psychological approaches to digital institutions have represented some of the biggest successes in prescriptive guides to building online communities \cite{Kraut:2012uk}. However, they tend to focus less on the effects of users on the institution, with a more single-minded effect of the institution on users, as in e.g. studies of interface effects \cite{Restivo:2012km, Gallus:2015ux,burghardt2016myopia,Forderer:2017vz,krafft2018experimental}. Several other subcommunities of social psychology have studied the performance and health of digital institutions with a focus on their effects on individual behavior. Team behavior researchers have established the importance of ``psychological safety'' for team success \cite{edmondson1999psychological,duhigg2016google}. Researchers studying collective intelligence have investigated factors that lead to good generalized coordination and collaboration abilities in teams \cite{woolley2010evidence,krafft2015emergent,kim2017makes,krafft2018simple}.  
% \item[Economics.] Economics is by far the dominant normative and prescriptive framework for reasoning about incentive structures, which is critical for digital institutional design. Several researchers have applied game theoretic framings to emergent digital institutions in multiplayer games \cite{Cavender:2013bm,Ross:2014wc,Ross:2012dw,Strimling:2018vf,Castronova:2006kn}, especially digital market institutions \cite{Salter:2013ed,Castronova:2009is,Hardy:2016cr}.  
% \item[Human computation.] Researchers in human computation study both mechanisms for crowdsourcing (e.g., \cite{lasecki2013warping}) and also topics such as interface design decisions informed by game theoretic considerations \cite{dash2003computational,mao2013better,chen2016mathematical}.
% \end{description}


%All of these frameworks are useful, but the Ostrom  subsumes many of them and adds more besides. \sf{\pk{Describe the unique benefits of the Ostrom . Don't sell as ``best'' but as adding unique value. No need to discuss limits of other frameworks in this case.} Unfortunately, these contributions have contributed to the somewhat fractured pattern by which social theories are brought to bear on the challenges of computer supported collaborative work. Drawing from a body of work that endeavors to integrate cultural, economic, and political perspectives, we Our contribution build integrates of theory. }

%\subsection{Alternative frameworks}
%Does the problem of digital institution design really demand another framework?  There are many alternatives---org theory, social networks, social psychology, game theory, and more---that have been used to study digital institutions.  Nevertheless, these frameworks all fall short of the requirements of a satisfactorily complete science of digital institutions.
%\subsubsection{ Organization Theory.}
%The resource management paradigm is most comparable to that of organization theory (``org theory'').  
%Org theoretic studies that have shed light on digital institutions are the most likely to have a strong sociological flavor, and they 

%Still org theory has several shortcomings as the basis of a science of digital institutions. It is traditionally focused on just one type of institution---businesses operating within a capitalist socioeconomic framework---and, despite a decades-long tradition of comparative work, comparative org-scale studies remain low-$n$, mostly qualitative, and have not taken advantage of the opportunities of the digital age. 
%In a resource system, agents' efforts to devise a scheme and coordinate with respect to it may well result in something that could be modeled as an organization, but understanding its effectiveness requires appreciating the disparate goals and incentives of  agents at all levels, the ecology of the resource, the mechanics and legitimacy of their scheme, and the specifics of their efforts to define, maintain, and evolve it with respect to resource conditions. From the socioecological perspective of the Ostrom Workshop, the organization is impossible to understand without equal effort to understand the resource that it is organized around. And as we will see, many problems of digital institution design are cleanly understood as concerning the efforts of autonomous agents united by a common resource constraint. 
%\subsubsection{ Social networks.} Understanding social systems requires taking the structure and function of social network into consideration.  The study of social networks has been an area of interest in sociology for a majority of the last century.  In this time sophisticated mathematical techniques for representing and analyzing social networks have been developed, and influential social theories relying on the logic of social networks have been articulated.  Social networks can help us understand small-scale social settings as well as organization-scale and societal scale settings. Social network theories have many other qualities required of a theory of institutional design: a history of interdisciplinary appeal, computational savvy, and interest in scalability, dynamics, and development. 
%Another popular framework is network science. 

%The primary limitations of social networks for institutional analysis are that this toolkit predominantly operates descriptively and not prescriptively, that its digital applications are more quantitative than qualitative, and that it is ultimately focused quite narrowly on questions of structure, at the expense of other important dimensions of institutional variability.  %While there have been some empirical studies of which network structures are better or worse for information flow, there are few well-understood design principles or normative standards.  Design is fundamentally forward-looking, and requires a framework that can advise on where to look for answers to design questions.
%\subsubsection{ Social psychology.}  

%A comparison of hundreds of peer-driven Q\&A communities on Stack Exchange investigated the effects of different affordances provided by the interface on stimulating quality contributions \cite{burghardt2016myopia} and increasing engagement \cite{Forderer:2017vz}.
%Experiments with randomly rewarded Wikipedia barnstars have shown improved productivity, retention, and identification with the community among rewarded editors \cite{Restivo:2012km, Gallus:2015ux}.

%Similar to research in social networks, this smattering of communities and results has is largely disparate and descriptively focused.  Social psychological approaches tend to focus on smaller scale social systems or narrowly constrained aspects of more complex systems, and they are less likely to complement their interest in individual-level effects with attention to system-level effects.
%\subsubsection{ Game theory and economics.} 

%The purview of game theory is broad, but one of the areas most relevant is mechanism design.  Mechanism design seeks optimal incentive structures, and ways to support implement those incentives, to achieve desired behavior.  While similar in aim to Ostrom's frameworks, game theory is more limited.  Game theory is based on an assumption of rational utility-maximizing agency, and there is little acknowledgment in game theory of human behaviors---such as social norms and cultural values---that do not fit neatly inside a rational agent model.  Game theory also considers fewer degrees of freedom in design than Ostrom's frameworks. For instance, there is no straight-forward syntax for reasoning about complex systems of rules in game theory, but systems of concatenated or nested game theoretic action situations are central to institutional design. Because of these limitations, game theorists tend to focus on smaller scale groups of people, or simple institutional forms such as markets.  
%\subsubsection{ Human computation.} 
%In computer science, the area of human computation is related to institutional analysis.    %Human computation tends to focus on small groups, interfaces for individual personal use, or problems whose scalability comes from their narrow scope and simplicity.


%\pk{Add a bit about multiagent systems approaches from CS?}

 %\section{Cases}

%\sf{Veto: \pk{Motivate need for framework by introducing our three case studies and the difficluties that people are having? (Describe in a pre-theoretic way)}  Brian and I still like Framework first.  Also, the upsides of an early dip into the cases has a downside of fracturing the Cases section in a way that is rough on readers. The cases below will be cleanly structured and much friendlier, which should give us another way to tackle the concerns that drove your suggestions}


% \begin{table}
%     \brian{Not convinced we need this}
%     \small
%     \begin{tabular}{p{5in}}
%     \begin{description}[leftmargin=1em]
%     \item[Resource.] Objects, virtual or physical, or value to independent agents in pursuit of individual or collective goals. Resources are commonly classified along dimensions of excludability, the ability to keep others from consuming the good, and subtractability, the ability of one's enjoying the good to reduce the ability of others to enjoy it (see Table~\ref{tab:goods_table}). Digital resources include time, attention, compute power, server space, and money. 
%     \item[Collection action problem.] A social outcome that negatively affects all agents, but that is produced by those agents' pursuit  of their  individual goals. Also referred to as a ``social dilemma.''
%     \item[Institution.] The prescriptions that humans use to organize all forms of repetitive and structured interactions by shaping individual and collective choice '' \cite{Ostrom:2005tg}. This very broad definition includes platforms like Facebook or Wikipedia.org, organizations like Microsoft or the Free Software Foundation (FSF), and standards like the Internet Protocol. Institutions may or may not be organized to manage a resource-driven collective action problem, but all require resources and are constrained by resource limits.
%     \item[Common pool resource.] A resource that is finite and cannot be privately owned (see Table~\ref{tab:goods_table}).
%     \item[Public good.] A resource that is infinite but cannot be privately owned (see Table~\ref{tab:goods_table}).
%     \item[Public bad.] A public bad is like a public good, except that it provides negative utility.  Digital examples include spam email and online harassment. Collective action problems typical of public bads focus on preventing their spread or remediating their effects. 
%     \item[Tragedy of the commons.] A type of collective action problem typical of common pool resources in which individually rational incentives to over-extract a resource produce scarcity for all. Digital tragedies include joining an overcrowded server, posting on a forum in which attention is scarce, or abusing a public wireless network.
%     \item[Public goods provisioning.] A collective action problem in which a freely accessible public resource suffers,  despite being effectively unlimited, because of the cost of maintaining or otherwise provisioning it.  Examples include failing to seed a torrent, to donate to a not-for-profit institution like the FSF,  to contribute edits to Wikipedia, or to host a mirror of a software project for downloading.
% \end{description}
% \end{tabular}
% \caption{Resource management vocabulary and examples.}
% \label{tab:vocabulary}
% \end{table}

%\subsection{The paradigm of the Ostrom Workshop}

%The work of the community around Elinor and Vincent Ostrom, known collectively as the Ostrom Workshop, is a political theory that understands political systems as things built by people, and that draws upon behavioral rational choice.  The former commitment, called methodological individualism, makes it natural to understand as a design theory, something rare in political science.  The latter commitment understands agents as easier to model as increasingly rational when they have a clear high-stakes goal, as is commonly the case in resource management dilemmas. But increasingly rational is still far from infinitely rational, and the theory understands resource system stakeholders as having limited reasoning and learning abilities, preferences for others, and values and emotions. Being focused on individualism, the Ostrom Workshop provides a micro-scale framework that understands governance in terms of the challenges that collections of stakeholders face in  managing finite resources and facing up to other problems of collective action.  It takes a governance view of collective structure, viewing social systems as much in terms of rules, norms, and endogenous contestation as in the more familiar terms of regular patterns of interaction and information flow.

%defend the novelty of this combination of different Ostrom frameworks

%\subsection{Institutional Design Challenge 3: Survivorship bias}

%\pk{Personally I think we should remove this challenge. It is of a different sort than the others.  It is a problem with analysis, not resource management.  Or at least that is how it is currently framed.}

%As surprising as the variety of successes is the magnitude of failure: successful communities are anomalies because the vast majority of communities are failures. Within an analysis of 300,000 Minecraft servers, only 150,000 ever responded to any of our hourly pings over two years, and only 90,000 were live for more than one month.  Within another sample of 5200 servers, we found that only 1800 ever received regular visits from  more than one user. The common practice of celebrating extraordinary design successes has brought considerable peril as we miss opportunities to learn from ubiquitous design failures \cite{Hill:2017tx}. Abraham Wald's counter-intuitive recommendation to reinforce the armor in undamaged areas of returning World War II bombers popularized the concept of ``survivorship bias'': the bombers returned because they were undamaged in sensitive areas~\cite{mangel1984abraham}. A \textit{population of populations} approach similarly enables comparative analysis of where to reinforce the design of institutions by learning from failures rather than patching insignificant areas.

%By conducting large-scale quantitative comparative institutional analyses over populations of successes and failures, we aspire to provide amateur server administrators, acting as dilettante political theorists, with the tools they need to come to collective action prepared, and to walk away from their first experiences of leadership with a track record of success. The resource management framework has the descriptive, interpretative, explanatory, and methodological richness that we require in order to define these communities around their key commonality, and credibly pursue our goal. 


% What of the successes?  Is there a key governance trait they share? , And among those that succeed, there is no clear unifying principle.  

%describe domain. what, e.g. does sucess mean? 

%most fail, those that succeed all do something different. how is it achieved: minicases. They they all have in can comprehend the idea of an administrator, the ideal fo a democratic server, of an excplicitly capatialist server. the closed off pristine server. 


%What is the appropriate faramework for asking thiese questions?  game theory falls short because the game is changeing, and becaus ehtere is a non-uniqueness problem. social nets fail for ther reson.  org fails because of competition dynamics. Furthermore, they vary dramatically in size. teams? orgs? states?  but resource constraints are the driver of success and failure.  

%advantages of ostrom: these differetn solutions seem irreconcilablely different: with each calling for a different framework, but why: they are all on the same platform, the same software, solving the same problem. tragedyof the commons provides a unifying frameowkr for these otherwise irreconcilably different insittutions. 
%This in turn, allows us to compare very different styles of governanments apples-to-apples.  In fact Ostrom already has a track record of applications to comparative :


%my own teaser findings. 

%\sf{NOT SURE IF THIS IS TRUE WITHOUT TWEAKS OF LANGUAGE, but worth adding if it is: The inflexibility of cryptocurrency's hard-coded approach to self-governance is evident in two other widely recognized symptoms of ineffective institutions. A cryptographic institution allows only a binary response to malicious users who violate the terms of a currency's smart contracts: they can either be tolerated with no punishment, or completely blackballed. Research in the resource management space has shown that systems are most effective that implement graduated sanctions, with a range of responses between the most tolerant and the most extreme \cite{XXX}. Informal norms can often help graduate an institution's formally harsh binary responses, but informal norms are less effective in systems like digital currencies that provide for anonymity \cite{XXX}.}% a second symptom of inflexibilty is the consensus requirement.  consensus doesn't scale, and requirement seems to belie the libertarian aspirations.}

%\subsection{Other stuff}
%\brian{I'm struggling to integrate the content below into existing sections or to label them as distinctive institutional design challenges}
%Further, even if market pressures are enough to drive currencies toward social optima, they have only succeeded at finding the optimum over the population of currencies.  For the community within a currency---each of whose agents has substantial investments at risk---finding satisfactory values of these parameters means building a ``trustfull'' political system outside of the trustless environment of the currency, with defined stakes, stakeholders, and the mechanisms of mediation and deliberation. As a cryptocurrency accumulates such a complicated institutional scaffolding, it gets bogged down by political problems it claimed to supersede, and its  distinctivness from traditional currency becomes increasingly muddled.


%Third, researchers have also documented evidence for manipulability \cite{} and historical large-scale manipulation \cite{} of cryptocurrency markets. \sf{NOTE:Pete, say that things are centralizing}. \sf{A well documented property of the resulting oligopolies and oligopsonies is the problem of cartelization, in which agents collude to gain control over a market and manipulate for their benefit.  This problem is as old as markets, with Adam Smith himself famously observing ``People of the same trade seldom meet together, even for merriment and diversion, but the conversation ends in a conspiracy against the public, or in some contrivance to raise prices.''  An example of this in cryptocurrency exchanges is the pump and dump scheme, in which many agents collude to raise prices, and then sell at the artificially high price.  Such cartels are interesting from a resource management perspective because they actually  show that  peripheral collectives of agents are profiting by  creating informal trustful institutions that help them overcome a resource problem.  Currency manipulation schemes set up tragedies of the commons, as the profitability of the scheme depends on the participants maintaining discipline, without any means of enforcement, and with increasing incentives to break rank and cash out.  The success of these cartels in the face of the Tragedies they should imply suggests that informal self-governing institutions can implement creative market manipulation schemes, both centralized and decentralized, that can undermine currencies by amplifying their volatility and decreasing trust in their ability to provide a solid foundation for economic exchange.}
 
 
%These considerations, whether definitive or open to further debate, highlight the highly political complexities of cryptocurrencies that are ignored under the cloak of ideology, and which institutional analysis as a field is oriented towards systematizing.







% \section{Case Study 3: Cannabis informatics}
% Information technologies play a crucial role in the regulation of emerging recreational cannabis markets. Recognition of the medicinal benefits, economic potential, and racial disparities in law enforcement have all contributed to a dramatic shift in attitudes and policy towards legalizing cannabis~\cite{Geiger_sixintenAmericanssupport_2018,schnabel2017should}. While states such as Colorado and Washington have operated regulated marketplaces for recreational cannabis since 2014, the production, distribution, and consumption of cannabis remain federal crimes that carry significant penalties. The legal rationale against federal intervention is the ``closed loop theory'' that requires demonstrating cannabis neither leaves the marketplace nor crosses state borders. 

% A central component of these new legalized markets are government-controlled ``seed-to-sale'' inventory auditing systems that collect and store detailed data about each transaction for every product to discourage ``diversion'' into untaxable grey markets or into legally-jeopardizing interstate trade. The instrumentation, collection, analysis, and reporting of data is pervasive in the industry in response to regulation, consumer demand, and investor pressure. The demand for, access to, and inferences from data influence decisions have significant financial, policy, and social value. Despite these seemingly strong incentives for actors in a precarious market to pool their data-intensive resources and to coordinate their behavior to secure a common good like ``multi-dimensional empirical proof of the harm caused by federal policy'', the collection, sharing, and analysis of data instead is instead falling into conventional institutional arrangements that are individually and collectively sub-optimal.

% %The design, implementation, and administration of the METRC system foreclosed on alternative possibilities for designing a new digital institution in the focus on this ``anti-diversion'' mission, but this system also was rapidly revised in response to multi-stakeholder participatory design to create a more effective system. This case will provide both an example of how digital institutions can fail without sufficient design consideration for all the actors who interface with them as well as how digital institutions can repair by employing participatory design processes.

% % An arrangement in which bipartisan political consensus, significant economic opportunity, desperately-needed social reform, and the shared commitment to data collection to legitimize their violation of federal law \textit{still} face collective action problems when designing digital institutions to collect and analyze their data, suggests the need for greater attention to the concept of digital institution design and their implications for overcoming collective action problems. 

% \subsection{Institutional Design Challenge 7: Surveillance commons}


% % \begin{figure*}[tb]
% %     \centering
      
% %     \minipage{.6\textwidth}
% %         \includegraphics[width=\textwidth]{images/it_components_parts.png}
% %         \caption{The ``IT component parts'' of the METRC system and its interfaces with different technologies and stakeholders.}\label{fig:it_components_parts}
% %     \endminipage \hfill
% %     \minipage{.3\textwidth}
% %         \includegraphics[width=\textwidth]{images/tagging_life_cycle.png}
% %         \caption{The ``tagging life-cycle'' of the METRC system.}\label{fig:tagging_life_cycle}
% %     \endminipage
% % \end{figure*}

% % \begin{figure*}[tb]
% %     \centering
% %     \minipage{.55\textwidth}
% %       \includegraphics[width=\textwidth]{images/tagged_plants.png}
% %       \caption{The RFID-enabled tags enabling the ``track and trace technology'' are attached to every plant in the statewide market's supply chain from seedling through vegetating, flowering, trimming, processing, transfer, and retail sale.}\label{fig:tagged_plants}
% %     \endminipage \hfill
% %     \minipage{.4\textwidth}
% %       \includegraphics[width=\textwidth]{images/scanner_screenshot.png}
% %       \caption{The scanner is used for entering data about the inventory, the data can be viewed and edited via a web interface, and this industry-collected data is read into a centralized database for regulatory monitoring.}\label{fig:scanner_screenshot}
% %     \endminipage
% % \end{figure*}

% The Marijuana Enforcement Tracking Reporting Compliance (METRC) system plays a central role in Colorado's \$1.5 billion cannabis industry. METRC is a ``regulatory compliance system'' licensed by the State of Colorado's Marijuana Enforcement Division (located inside the Department of Revenue) from Franwell, Inc., a privately-held, supply chain technology services company. All medical and retail marijuana businesses in Colorado are required ``to use METRC as the primary inventory tracking system of record''. METRC was built ``by regulators specifically for oversight'' to provide ``the necessary visibility for adherence to rules, regulations and statues'' to fulfill the legal demands of the ``closed loop theory''\footnote{https://www.metrc.com/the-system}. Figure~\ref{fig:it_components_parts} shows METRC's two sides: an industry side that is ``used to report the required events and information'' and a regulatory side is ``used for enforcement and compliance monitoring''\footnote{https://www.metrc.com/the-system}. The industry side consists of RFID-enabled tags and barcodes attached to the plant and its derivative products that track them through the market ``from seed to sale'' (see Figure~\ref{fig:tagging_life_cycle}): this involves tagging seedlings and clones, vegetating and flowering plants, trimmings, business-to-business transfers and distribution, and final sale at a retail location. The inventory and status is entered with specialized tag scanners and web user interfaces (see Figure~\ref{fig:scanner_screenshot}) into a central database. As Figure~\ref{fig:it_components_parts} shows, METRC allows regulators to perform live audits to trace provenance of every single product in the state-wide marketplace using METRC's own reporting tools within itself or by using METRC's APIs to pass its data to secondary and tertiary data analysis systems. 

% The medical and recreational cannabis markets are examples of ``polycentric governance'' involving many centers of regulatory authority and the mutual \textit{interdependence} of these jurisdictions' decision-making: state-level legislators craft policy around federal-level legal memoranda while preserving the autonomy of local-level jurisdictions to issue licenses to operate. These multiple levels of governance potentially allow the multiple sectors impacted by this market (regulators, entrepreneurs, consumers, activists, journalists, researchers, \textit{etc}.) to engage in rulemaking, market production, monitoring, and sanctioning. However, METRC undermines the potential of this polycentric system because its data collection and auditing model is centralized at a single level (state regulators), for a single function (inventory audits), in a single sector (public safety and revenue). 

% The capture and enclosure of previously unmanaged data into these tracking and auditing systems mirrors other threats to the possibilities collectively owned and managed knowledge in these new markets. Despite some superficial similarities such as pooling private data into a public agency's database, METRC mirrors more of the institutional logics like Zuboff's ``surveillance capitalism'' that combines the power of new digital systems with extractive business models and unaccountable governance~\cite{zuboff2015big}. Rather than creating a knowledge commons that would enable different market participants to make use of the pooled and valuable data, this data is pooled into a commons for surveillance and enforcement purposes with little value reciprocated from the state back to producers, consumers, or other polycentric authorities. We might call this a ``surveillance commons'' in which knowledge is shared with a public agency but enclosed and unavailable to other participants.   

% %It is worth acknowledging on what a remarkable socio-technical achievement a centralized, industry-wide inventory tracking system like METRC is. In the early 1970s, the Salvadore Allende administration in Chile implemented ``Project Cybersyn'', a distributed decision support system for monitoring and managing the national economy through a network of data collection feeding into a centralized mainframe~\cite{Medina_CyberneticRevolutionariesTechnology_2014}. METRC has a similarly ambitious scale of individually-tagged plants (Figure~\ref{fig:tagged_plants}) and specialized scanners and web interfaces for feeding inventory data into a central government database (Figure~\ref{fig:scanner_screenshot}). Unlike Project Cybersyn however, METRC was designed to protect the privacy of those submitting the privileged data it collected. 

% \subsection{Institutional Design Challenge 8: Path dependencies and network effects}
% The adoption of METRC in response to the animating ``closed loop'' legal theory foreclosed alternative institutional designs: a supply chain problem demanded supply chain solutions. METRC has some compelling parallels with the Allende-era ``Project Cybersyn'', a distributed decision support system for monitoring and managing Chile's national economy through a network of data collection feeding into a centralized mainframe~\cite{Medina_CyberneticRevolutionariesTechnology_2014}. Both Project Cybersyn and METRC operate from similar logics of top-down, centralized command-and-control prioritizing specific variables to be measured and collected in data formats defined by regulators to compatible with their modelling approaches and political interests. Because every business in states' regulated cannabis market are required to maintain plant-level data, METRC implements a ``secure reporting environment'' for industry participants where they can ``access their own data but no other participants' data'' but the regulator has ``access to all industry participants' data.'' The collection of detailed, timely, and valuable data into a centralized database required regulators to provide privacy affordances under the assumption that private market actors would use their competitors' data reporting against them.

% %The design and implementation of a centralized government database of an entire industry's inventory with strong privacy guarantees was a political decision made from a set of assumptions about how market actors would defect rather than cooperate given the opportunity to access vital industry data. 
% % collective interests, individual motivations, business models, social problems, and technological capabilities

% Cooperative models were popular models in the cannabis markets predating recreational legalization: patient would give their state licenses to grow medical cannabis to third-party cooperatives who supplied the flower product back to the patient~\cite{feldman1998providing,dioun2017making}. In the black market, cooperative models were also used by illicit organizations as a form of mutual aid in the absence of access to traditional risk management and dispute resolution strategies like insurance, banking, accounting, and arbitration~\cite{sandberg2012importance,moeller2015credit,moeller2017debts}. Legalization introduced ``white collar'' private equity investors and management consultants whose capital and operational expertise has increasingly displaced the ``green collar'' enthusiasts and activists whose political organizing secured legalization policies. Despite the strong incentives to pool knowledge resources and coordinate behavior to stabilize a precarious market, actors restricted access to large-scale and standardized data in the name of ``privacy'' to prevent competitive information arbitrage among market participants. Alternative mechanisms for production, exchange, and coordination could have (and did) exist, but the lack of conscious institutional design introduced path dependencies precluding coordination and information exchange while rewarding private returns and siloed data.

% A related form of path dependency also exists in the form of network effects around the adoption of inventory tracking as a regulatory model and the adoption of the private systems to implement this tracking. Franwell, Inc. (the developer and owner of METRC) offers ``internet-deployed applications and services'' and ``RFID technologies'' improve ``track and trace visibility'' for perishable foods, pharmaceuticals, and (not stated on their website) the state-mandated cannabis inventory tracking systems for the medical and/or recreational markets in 10 states. Franwell, Inc.'s METRC competes with other platforms like BioTrackTHC to secure the contracts to implement each state's inventory tracking system, but its early adoption by the first states has made it the technical standard for newly legalizing state regulators averse to the risks of newer, smaller, and untested inventory tracking systems. This is a network effect because the value of the service increases with the number of adopters: the widely-adopted system becomes more reliable and usable as well as can set standards for compliance and interoperability. The absence of conscious digital institution design again contributed to outcomes that concentrated benefits while distributing costs.



% %This zero-sum competitive market dynamic undercuts the trust necessary between these social groups to cooperate to secure further greater regulatory concessions to enable them to grow. 

% %Despite these cooperative antecedents, the legalization of recreational consumption has embraced investor-driven corporate models relying on specialized mass agriculture, operational specialization, and brand marketing to preserve the financial margins after wholesale prices plummeted as supply in the marketplace increased. Put another way, the 

% %\brian{displacement of alternative models of production, what alternatives could have existed, can still exist?, sharing more data to secure better individual and collective benefits}
% % But an institutional analysis suggests that alternative rules for the boundaries, positions, choices, payoffs, scope, aggregation, and information rules could and did exist.

% \subsection{Institutional Design Challenge 9: Multi-stakeholder iteration}

% Because the legality of these markets centers on a provenance problem with supply chain solutions, the implementation of this digital institution initially assumed the recreational cannabis market could be translated from solutions for perishable foods or pharmaceuticals. This top-down isomorphism assumption had a lack of congruence with local conditions: it did not account for the multiple stakeholders, unique regulatory constraints, and alternative business models specific to the cannabis industry's needs for a minimally-functional digital institution. METRC was initially ill-prepared to fulfill the market demands: it did not manufacture enough RFID tags, the central database had poor usability and reliability, and innovative new products and business models did not fit into METRC's models for logging inventory data and transaction events. The supply chain solution did not initially solve the problems of designing a digital institution for regulating a legally precarious marketplace.

% In a remarkable turn for government information technology deployment, the multiple stakeholders interfacing with METRC committed to a participatory process for revising the design of the system. Growers, retailers, regulators, technologists participated in a series of meetings to identify the fault lines between the legislatively-mandated affordances, rules-in-use, and emerging practices. A significant development was the introduction of a more robust API that allowed METRC to fulfill its statutory obligations to be a central inventory tracking system while also providing producers and retailers greater flexibility to develop alternative approaches for entering, representing, and retrieving data with secondary and tertiary systems. This API currently has end-points for employment, facilities, harvest, items, lab tests, packages, patients, plant batches, plants, rooms, sales, strains, and transfers: a panopoly of data instrumentation that could not have been anticipated coming from supply chain models of perishable foods or pharmaceuticals.

% Although this effort to repair the ill-designed system did not change other institutional configurations around regulatory requirements, concentration of data, or graduated sanctions, it did show commitments to design for congruence with local conditions, incorporating collective-choice arrangements, and experimenting with conflict-resolution mechanisms. The importance of having a \textit{legitimate} digital institution to justify the precarious legality of a new and high-profile market was an instance of successful digital institution design insofar as the institution could be repaired in the absence of prior precedent or formal constitutional mechanisms. 

%\subsection{Institutional Design Challenge 10: Surveillance commons}
% From a resource management perspective, govt database, small practitioners, they all share resource problems of contributing to knowledge commons



%The ability to repair a flawed design in a digital institution suggests these repairs could be extended to support other collective goals among market actors, government regulators, and civic actors. Despite the desire by policymakers and regulators to track the provenance of products through the entire market, these data are characterized by a lack of standardization, interoperability, and exchange between market actors (customers, farmers, retailers, investors, \textit{etc.}), government actors (policymakers, law enforcement, tax revenue, public health, \textit{etc.}), and civic actors (journalists, researchers, activists, \textit{etc.}).

%A major challenge is the lack of a standard for uniquely identifying strains. The primary psychoactive cannabinoid THC, the non-psychoactive therapeutic cannabinoid CBD, as well as non-cannabinoid terpenes that impart \textit{cannabis}'s distinctive smell all appear to have main and interaction effects on bio-availability, physiological effects, and subjective experience of cannabis consumption~\cite{GrotenhermenMedicinalUsesMarijuana2016}. Much as beer menus now report the alcohol by volume (ABV) and International Bitterness Unit (IBU), cannabis companies breed, test, track, and market for an increasing number of chemicals beyond the state-mandated THC concentration reporting. The lack of standardization produces a situation where multiple strains, all branded ``Girl Scout Cookies'', can have significantly different genetic and chemical compositions: something called a Heineken could not only end up being a Budweiser or Corona, it could also be a Guinness.



% Come in at beginning physical institutions mediate digital interactions
% A framework to understand bureaucracies, capitalized markets, black markets coexit
% Are there tacit norms in the database itself or interpretations of how the database should be designed or used
% Ostrom on municipal police departments, polycentricity of sharing a crime lab, some cities have centralized versus decentralized decisions about where officers patrol regularly versus rotating through an entire city, crime labs should be centralized to be more effective, what makes sense to centralize or de centralize: polycentricity and federalist/nested system can be organized highly centrally versus distributed
% technology foreclosing alternatives: farmers in Nepal
% repairs: populate the ostrom framework with the cannabis informatics case, "design something that follows these rules and it will work", "diagnose your existing institution's problems with this list", increasingly participatory framework from low level stakeholders representing in high-level decision making, growers and cooperative models represented versus being hedged out

%\brian{Other parts of the digital institution besides METRC: banking, taxes, finances, postal, access to advertising platforms, crime reporting, Healthy Kids Colorado; extending lessons from repair of digital institutions to solve other collective action problems around lack of standardized data formats, exchanges, models to drive policy change more aggressively}


% \begin{table}[tb]
%     \footnotesize
%     \centering
%     \begin{tabular}{lrp{3in}}
        
%         %\multicolumn{2}{c}{Framework elements} \
%         \textit{Component} & \textit{Element} & \textit{Example} \\
%         \toprule
        
%         \textbf{Technology} &METRC& \emph{A supply-chain monitoring solution originally designed for government monitoring regulatory compliance of pharmaceutical producers} &\\
%         \textbf{Roles} & \emph{Producers} & Growers, manufacturers, and other agents on the cannabis supply chain\\
%         & \emph{Regulators} & State agencies responsible for licensing, compliance, and enforcement\\
%         & \emph{Monitors} & Firms that maintain supply chain tracking infrastructure\\
%         & \emph{Consumers} & Cannabis consumers \\
%         [3mm]
%         \textbf{Resources} & \emph{Cannabis products} & Private good. Seeds, plants, and other components of cannabis products tracked through supply chain\\
%         & \emph{Taxes} & Public cost. Collected from consumers to support regulation efforts.\\
%         [3mm]
%         \textbf{Rights} & \emph{To enjoy} & Consumers \\
%         & \emph{To extract} & Producers \\
%         & \emph{To buy/sell} & Producers, constrained by regulators \\
%         & \emph{To manage} & Regulators, constrained by law \\
%         & \emph{Meta-rights} & Regulators and state legislative apparatus. \\
%         [3mm]
%         \textbf{Rules} & \emph{State} & Laws and policies define interactions between agents in the different roles.\\
%         [3mm]
%         \textbf{\makecell[tl]{Rules \\by level}} & \emph{\makecell[tr]{Operational layer}} & Laws and policies define possible actions. These differ by state \\
%         & \emph{\makecell[tr]{Collective action layer}} & Consumers and producers are excluded from collective action layer, except through political channels such as lobbying. \\ 
%         & \emph{\makecell[tr]{Constitutional layer}} & Determined by state's legislature, with some rights to regulators. Role of state makes constitution-level change slow and difficult \\[3mm]
%         \midrule\\
%         \textbf{\makecell[tl]{Resource \\challenges}} & Resource processing & State capture. System designed for narrow range of cannabis products (flowers), in a way that inhibits trade in more processed goods (oils, resins, food products, etc).\\
%         & Institutional incongruency &State capture. Requirements on resource use and management are orthogonal to consumer requirements because resource is tracked like a medical product but primarily used recreationally \\
%         &High costs&State capture. Cost of regulatory apparatus in taxes and compliance keeps legal product above pre-legalization prices\\ 
%         %&Barriers to entry&Highly regulated atmosphere selects against small agents and unfamiliar models\\
%         %&Path dependency&Because system has precedent, it spreads in a way that perpetuates early bad design decisions\\
%     \bottomrule
%     \end{tabular}
%     \caption{Specification of the cannabis informatics case from a resource management perspective}
%     \label{tab:summary}
% \end{table}%\vspace{-3em}


%\subsection{Social Media}

%\sf{NOTE: this might be getting there.  I don't see it yet.  here are two (commented out) leads/links that might help. they illustrate Lin's (conceretd) efforts to integrate the sociological theory of social capital with her own frameowkrs for understanding institutions empirically:
%https://books.google.com/books?hl=en&lr=&id=6PZ8bvQQmxEC&oi=fnd&pg=PA172&dq=%22social+capital%22+ostrom&ots=EIkgycbMYh&sig=Q-RYOJVsjs2uIhu2pU5zV5nACNU#v=onepage&q=%22social%20capital%22%20ostrom&f=false
%https://books.google.com/books?hl=en&lr=&id=fOMUwqb9AIUC&oi=fnd&pg=PA17&dq=%22social+capital%22+ostrom&ots=UzXBPWLYxK&sig=J8l5rzKY4HiwkWPPNF8jFpE1U_I#v=onepage&q=%22social%20capital%22%20ostrom&f=false


%As our final example we examine the structure and role of Facebook.  Facebook operates internally predominantly as an advertising platform, but Facebook also manifests in people's lives in more complex ways.  As a space for community, Facebook has some relationship to traditional institutions such as religious centers, coffee shops, public parks, and other gathering places.  Facebook functions as what sociologists call a ``third place''---a social space separate from one's home or workplace.  

%One of the fundamental resources of community in a third place that must be both created and sustained is social capital.  Architecture---whether physical architecture or software architecture---unavoidably creates an implicit institutional / regulatory frame that impacts the shape and strength of social capital.  In the case of physical architecture, this frame includes aspects such as who is likely to be in close physical proximity to whom, which has been empirically shown to have an enormous impact on patterns of interaction \cite{}.  How big are the tables in a coffee shop?  How easily can they be rearranged?

%Churches, libraries, town halls, parks, and many other publicly accessible venues in the United States dedicate significant square footage to large open spaces.  Open space is desirable from the perspective of community building because it allows people to fill that space with whatever they deem appropriate for a particular event.  Complex political systems become increasingly necessary as the size of a community increases, but third places, usually dealing with smaller communities, operate by providing open space for self-governance rather than dictating or regulating the interactions in that space.  They provide literal and metaphorical space for self-organization and self-governance. Facebook as a third place lacks such a capacity.

%Proximity and space management in the digital case involves the direction of attention through interface decisions.  Many web forums create third places that are more analogous to the traditional institutional form by allowing participants to create threads and interact in those threads, with peer moderation.  Facebook instead encourages wide-reaching unfocused interaction that is managed not be self-organization but by Facebook's organization.  This level of fine-grained control goes beyond what has been possible in traditional third places.  Facebook literally determines whose messages and what types of content attain preference in visibility.  The claim that Facebook makes it that these attention management decisions are for your own benefit, based on your revealed preferences, but this system both neglects your own goals that Facebook might not be able to infer and is susceptible to Facebook's own incentives as an advertising company.

%To put it mildly, the impact of these choices on community health and social capital is poorly understood.  Social capital relies on complex networks of social interaction.  When Facebook completely censors posts or certain categories of content, or simply reorders messages in your feed, it is explicitly paternalistically influencing the shape of our social networks.  Imagine if Starbucks was the only coffee shop in the world and the CEO of Starbucks implemented policies constraining who you could and could not talk to there, and what you could and could not talk about.  Due to the global reach of Facebook, its engineers are effectively unelected politicians practicing institutional design. Facebook governing with a red fist undermines the capacity for people to participate in self-organization, with unknown consequences not just for the ``Facebook community'' but also for our relationships with each other and the health of the world.  


%\sf{From the perspective of the resource managemnet view, what is trumpeted as the sharing economy, is little more than an application of technology toward expanding the market distribution of resources that institutional designers should aspire to distribute through more democratic, diverse, and creative digital institutions.}

%In the past, third places have been spaces for self-organization and community building.  





%\sout{ Tech entrepreneurs are therefore effectively unelected practitioners of institutional design.}





%In this capacity, the central questions of governance in Facebook are whether and to what extent the public sphere in Facebook should be regulated. 


%Resource of social capital as manifests in strong communities.



%he institution of the third place has historically often been a decentralized institution, at least in the United States.  In the United States, we do not regulate social interaction in coffee shops.  The major coffee chain, Starbucks, owns many locations, but Starbucks does not have a monopoly or near-monopoly on the coffee shop industry.  We have national parks, but most parks are small are locally managed.  

%Facebook in contrast is governed with a red fist.  Facebook engages in extensive censorship, further controls information flow by determining what content is displayed to you, and monitors all interactions it can observe---whether inside the platform or outside, as in for example your physical location and other websites you visit.  Facebook unilaterally makes changes to its system, without democratic process.  It is a mistake to believe that Facebook is accountable to its users because people can choose to protest or leave.  All authoritarian regimes are to an extent accountable to their citizens because regimes must avoid revolt. 

%Facebook as a third place in some ways mirrors historically public spaces that are becoming privatized.  Similar to a modern sports stadium or amusement park, Facebook assaults the consumer with advertisements while also tracking user activity to optimize it's profit goals.  Privately owned public spaces are regarded as more heavily surveilled and more carefully curated than publicly owned public spaces.  The justification for the privatization of public spaces is that the private authority has sole responsibility for maintaining the space.  Privatization avoids the tragedy of the commons in which nobody wants to invest in maintaining the public space.  

%Facebook similarly solves a maintenance problem.  Maintaining community requires a great deal of time and energy.  There must be people who create opportunities for interaction, there must be people who police community boundaries and norms to prevent harassment and other poisonous social interaction, and there must be people recruit new community members to offset attrition.  Facebook still relies on people to create content and recruit friends, but creates social incentives for content creation my making implicit social approval explicit in the form of ``likes'' and ``reactions''---both of which have been carefully designed to avoid negative emotions on the part of the content creator.  Facebook has taken a centralized solution to this maintenance problem in the sense that Facebook exclusively has control over how its platform is organized.  Looking to the literature on institutional analysis, we might be inspired to think about how to design Facebook to be more meaningfully self-governed.  A federalist structure is one interesting possibility.  Different groups of people have different desires and needs, and could tailor their digital spaces to those aesthetics like different coffee shops cater to different types of consumers---from people who enjoy a sanitized white-washed bourgeois hipster aesthetic to those who enjoy a dirty dingy basement aesthetic.  

%Such a system could involve rights to organize around proposing and responding to design changes (more so than lip service of a user forum or a ticketing system --- because these solutions still treat voting unit as the individual).  Perhaps Facebook could implement a liquid democracy to elect user representatives that advocate for particular design decisions.  Facebook currently varies from region to region, but this variance should be transparent and not out of management convenience but as an organizing principle for localized community participation.  If Facebook is to live up to its mission statement of truly fostering community, then we should not settle for the community of a Soviet Union but the community of a grassroots cooperative. 









%\section{CUT? Discussion}


%Towards more generalizable social science from online social behavior by doign comparative institutional analysis of different platforms

%Suitable for maybe for an ethics section: [Defense of Prescriptive] There are legitimate concerns among academics about any attempt to turn societal design into a science, or worse, a discipline of engineering. To presume to design a society that will behave as designed, that will not run afoul of the law of unintended consequences, is hubris. But if such hubris doesn’t appear from within communities that better, it will appear from those that don’t. Already, the dominance of a few firms over both the Web and the Internet, and the dominance of certain catchall design patterns, such as markets and hierarchies, is a deviation from the vision of the Internet as a tool of personal and community empowerment. Serving the people whose experiments resist these trends alternatives means moving beyond a description of their shortcomings to a procedure they can follow to increase their chances of success.

% Make sure to exhale, bruh
%The way society is tells us almost nothing about the way society could be.  We are allowed to be optimists.  But we must be steadfast in our night's watch.  We must pay careful attention to the cracks we see in the pavement along the road to our future society, lest our brave new world revisit the sufferings of our past or reimagine a way to new hells. The future is dim.  The future is bright. 

\begin{comment}
    *Our digest of the framework is tailored to digital designers
    *Successes of framework\\
        **Micro to macro\\
        **   Comparisons across cases\\
            ***     both minecraft and crypto cases have market for
            tyrants\\
            *** despite one being market driven, and one being state driven (despite being literally on opposite end of political spectrum, and ideologically opposed), both crypto and cannabis institutions have highly constrained institutional layers
        **Embrace economics while maintaining prominence of cultural\\   and political factors\\
            ***Specifically, we capture how technological, cultural, political, and economic dynamics interact.
                *** in Minecraft case, a constraint imposed by the technology creates an economic route to political change. in contrasts to an autocrat in a physical state, an administrator of a server on the Internet no in-game mechanisms for physically coercing users to stay. They may still have psychological and even economic leverage, 
                *** in cannabis market, we identify the economic effects of cannabis attaining its cultural role as recreational via a path through a legal role as a controlled substance and then a political role as a medical one.
                *** In crypto case, this framework makes it possible for us to pinpoint the weaknesses of using strictly economic mechanisms to implement an inherently political  system.
                *** The power of this integration has clear design implications: in markets for tyrants generally, cultural preferences for one over another set of values are driven to have a political effect of driving institutional change
                 
    *MAYBE: Comparison of resulting in\\
    
    * Four nodes all the same, ordering or structure of relationships between them different for each case
    * Different patterns of interactions has implications for design, because of constraints with different hand-offs, different flows, maybe they circle back or have non-sequential relations, constraints at each step
    * Suggest different flow for each case, emphasize the nodes but create a vocabulary for talking about different configurations of sequences
    * What kinds of contrainsts or discipline should be imposed on this flow/sequence approach so that everything isn't connected to everything or alternative permutations
    * Can concede everything causally implicated in each other, but some stronger than others, it's not impossible for 
    * Use nodes and arrows to narrate each of the cases
    ** Minecraft: Technology --> Economics --> Culture --> Politics
    ** Blockchain: Culture --> Technology --> Economics --> Politics
    ** Cannabis: Culture --> Politics --> Technology --> Economics
    * What are implications of different sequences?
    * Strongest claim: integrated tech-econ-cult-pol approach is important tells you what kinds of governance and management to design for
    ** If this, then that: still not holy grail of proscribing specific institutional choices.
    * Kinds of goods, kinds of sequences, kinds of governance.
    * Technology tends to make centralization more centralized, decentralization more decentralized. Creating/expanding a vocabulary to make more kinds of institional arrangements possible
    * Technology can help more kinds of institutions work for different resource types
    * Cultural constrain determining an institutional form: value of trustlessness and maximizing freedom at expense of other values
    * Weaker claim: We can anticipate problems with this integrated approach, problems if we had only taken a tech, econ or cultural angle we would have missed, 
    * It's about time we got some benefit from having engineers for reviewers


% \begin{table}[tb]
%     \small
%     \centering
%     \begin{tabular}{llc|c|c|c|c|c|c|c|c|c|c}
%         & & \multicolumn{11}{c}{\textbf{Design principles}} \\
%         \textit{Case} & \textit{Design challenge} & \rot{\textit{User boundaries}} & \rot{\textit{Resource boundaries}} & \rot{\textit{Congruence with local conditions}} & \rot{\textit{Appropriation and provision}} & \rot{\textit{Collective-choice arrangements}} & \rot{\textit{Monitoring users}} & \rot{\textit{Monitoring resources}} & \rot{\textit{Graduated sanctions}} & \rot{\textit{Conflict resolution}} & \rot{\textit{Right to organize}} & \rot{\textit{Nested enterprises}} \\ \toprule
%         \multirow{3}{*}{\textbf{Minecraft}} & Marginal cost management & \OK & \OK & & & & & & \OK & \OK & \OK & \OK \\
%         & Reification of folk theories & \OK & \OK & \OK & \OK & \OK & \OK & \OK & \OK & \OK & \OK & \OK \\
%         & Survivorship bias & \OK & \OK & \OK & \OK & & \OK & \OK & & & \OK & \OK \\ \midrule
        
%         \multirow{3}{*}{\textbf{Bitcoin}} & Sustaining altruistic monitoring &  & \OK & & & \OK & & \OK & \OK & & & \\
%         & The fact of politics & \OK & \OK & & & & & & & & & \\
%         & Engineering constitutions & & \OK & \OK & \OK & \OK & \OK & \OK & \OK & & & \\ \midrule
        
%         \multirow{3}{*}{\textbf{Cannabis}} & Surveillance commons & \OK & \OK & & \OK & \OK & \OK & \OK & \OK & & \OK & \OK \\
%         & Path dependencies & \OK & \OK & \OK & \OK & \OK & \OK & \OK & & & & \OK \\
%         & Multi-stakeholder iteration & \OK & \OK & \OK & & \OK & \OK & \OK & & \OK & & \OK \\
%         \bottomrule
%     \end{tabular}
%     \caption{Design principles (columns) implicated by the nine design challenges (rows). }
%     \label{tab:summary}
% \end{table}%\vspace{-3em}

\begin{figure*}[tb]
    \centering
%    \minipage{.4\textwidth}
      \includegraphics[width=\textwidth]{images/Comp_fig.png}
      \caption{Interaction between technological, cultural, psychological/economic, and governance factors produces collective action challenges for diverse digital institutions. \sf{ROUGH SKETCH. Replace with figure BK is drafting. ref: \pk{Add a box or a table that summarizes the implications of discovering a particular type of resource, right etc. include citations to what failures occur when implications are not considered, and what successes occur when the implications are followed}
}}\label{fig:scanner_screenshot}
 %   \endminipage
\end{figure*}


\pk{Replace with comparison to how other frameworks would have decomposed cases}



The three case studies illustrated the diversity and complexity of challanges that confront designers of new digital institutions. Minecraft server administrators have to manage the marginal costs of every new user and the plugins and other tools they adopt to do this management reify some folk theories of resource management to mixed effect, but the sovereignty of these servers provides a compelling \textit{population of populations} to avoid the survivorship bias that typically plague making inferences only from successful communities. Bitcoin remarkable success reflects a combination of technical implementation with first-order incentive design, but nevertheless is confronting existential governance questions around declining monitoring, the inescapability of political interests in decision-making about institutional change, and the importance of engineering constitutions that support efficient conflict resolution and and collective choice mechanisms. Finally, the legalization of state markets for cannabis critically depends on digital institutions for tracking inventory in the entire market, which has had the effect of creating a surveillance rather than knowledge commons, introducing path dependencies favoring some business models, but also providing models for cooperative problem solving in the face of existential threats to the system's legitimacy.

\sf{This leaves with mention of design principles elsewhere: ``Table~\ref{tab:summary} summarizes how different design principles (columns) from are implicated (positive or negatively) by each of the design challenges identified in the three case studies. Each of these digital institutions faces distinct serious, even existential, challenges that involve failures or repairs by multiple institutional design principles. In light of the pervasiveness of institutional design challenges across these diverse cases that involve more than one design principle, we return to our motivating question of ``why do we not design better digital institutions?'' ''}

With more general theories, that permit more ambitious comparisons of more superficially incomparable institutions, we get closer to a science of digital institution design that is general enough to avoid the problem of defining away from consideration the future's most creative, innovative, and inspiring experiments in digital institution building.  The best candidate for such a theory is the Ostrom Workshop's vast body of scholarship on the design, analysis of resource management institutions and the socioecological system in which they are embedded. It should be no surprise that the resource management paradigm is a natural fit for the CSCW community.  Frameworks from both have provenance in early computational theories of organization, in particular the cybernetics of Ashby \cite{Ostrom:1995vn,Bannon:1989va,Malone:1990cs,Jackson:2014ho}
with its focus in the structure of emergence and the mutual construction of institutional structure and agent behavior. 

The power of the Ostrom Workshop for digital institution design is evident not just in its fifty-year track record of producing transformative insights about self-governing institutions---from listservs and free software collaborations to international treaties governing the Pacific Ocean and self-governing irrigation networks in Nepal--- but also in the number and variety of classic or fundamental scientific divides it succeeds in bridging.

\subsection{Epistemological divides}

\subsubsection{The design/understanding divide} The demands that an engineer places on a theory are different from those placed by a scientist. For example, engineers tend to use models for prediction, while those seeking understanding more often use them to understand mechanism. Ostrom Workshop frameworks were developed by both scientists and practitioners with the needs of each in mind.  The IAD framework has this commitment baked into its name, as a tool for Institutional Analysis and Design/Development.

\subsubsection{The reductionist/holist divide} A science of design must be constrained enough to guide decision making and aid analysis, but must also be rich enough to allow for emergence, and for products that are at least as complex as they environments they must endure. Being built on ecologists' understanding of natural resource systems, the resource management perspective appreciates the everything-affects-everything nature of social and cultural dynamics, while allowing that some things affect everything more than others.


\subsection{Disciplinary divides}
\subsubsection{Qualitative-quantitative divide} From a scientific perspective, the work of the Ostrom Workshop is most notable for making it possible to perform quantitative falsifiable analyses of  seemingly intractable constructs like social institutions, community associations, and political self-organization.  But Lin Ostrom's training was in qualitative fieldwork, and Vincent Ostrom was a political philosopher. Consequently, the strategy they introduced for accumulating knowledge about social phenomena gave historical analyses and observational description a privileged position as the source of fodder for subsequent investigations to isolate and analyze, by formal models, lab experiments, and econometric methods. 

\subsubsection{Disciplinary divides} The findings of the Ostrom Workshop are one of the most important successes of interdisciplinary social inquiry in the 20th century, and they would not have been possible had the Ostroms not cultivated a culture that made scholars feel welcome and productive from political science, economics, anthropology, psychology, sociology, communication, organization theory, philosophy, and information science.

\subsection{Theoretical divides}
\subsubsection{The rationalist/social constructionist divide} While it is more tacit than political in the CSCW community, there is a clear divide between those who understand people as fundamentally sensitive and culturally contingent, and those whose agents start more or less economically rational. While both perspectives can allow the merits of the other, there are few clear strategies for directing these alternative perspectives toward integrated insights. Starting at the fact of the ``Drama of the Commons'' the Ostrom Workshop nuances a boundedly rational agent with sensitivity to history, culture, and others. It reconciles rationality with constructionism by understanding people as being transformed by the institutions that their ancestors built, and that they maintain and adapt.

\subsubsection{The unit-of-analysis divide} Scale has always been a satisfactory first-order organizing principle for the social sciences, as we move up from neurons to individuals, teams, groups, organizations, and states.  The information sciences continue to respect these divides, having contributed little to a multi-scale theory of social phenomena that holds the smallest groups and the largest organizations in the same embrace. As the social information sciences gain the ability to compare across populations whose populations differ by orders of magnitude, the need for such generality will become urgent. The resource management perspective provides just such a multi-scale theory, not in two senses.  The more minor sense is that it has been successfully applied to analyzing the effectiveness of small independent teams, large international treaties, and virtually every level of analysis in between.  The stronger sense is that it's frameworks make populations of 2 and 2000 comparable in the same study. And in the process, it gives us an unprecedented opportunity to pose questions about institution design were only recently impossible to pose, as multi-scale studies that once involved decades of data collection now take months or days. 

\subsubsection{The online/offline divide}  This last divide is not so apparent outside of the information sciences, in which prominent theories avoid discussing humans-most-generally-construed, or even go further to argue for the aspects of digital sociality that have nothing to offer the non-digital social sciences. By studying computer users instead of humans, we are missing unprecedented opportunities to bring new levels of rigor and new kinds of perspectives to each of the traditional social science's fundamental questions. By framing itself around resources most generally construed, the Ostrom Workshop brings digital commons into the already-diverse fold of physical natural resource commons, and puts computational scholars in a position to benefit, and benefit from, insights about human collective action that can fuel all disciplines. This work provides a path, if anyone wants it, for CSCW to move from understanding humans with technology to humans despite technology.


\end{comment}

 




%Institutions still a frontier
%Institutional work remains ununified
%Institutional framework unifies
%Comparative institutional analysis and MIIs for cross-platforms

%\subsection{Types of resources}\label{sec:types_of_resources}

% \begin{table}[tb]
%     \small
%     \centering
%     \begin{tabular}{llll}
        
%         & & \multicolumn{2}{c}{\textbf{Subtractability}} \\ 
%         & & \textit{Low} & \textit{High} \\ \toprule
%         \parbox[c]{2mm}{\multirow{11}{*}{\rotatebox[origin=c]{90}{\textbf{Excludability}}}} & 
%             \multirow{4}{*}{\textit{Difficult}} & 
%                 \parbox[t]{1.5in}{\textbf{Public Goods} \\ Radio stations \\ Wikipedia articles \\ Sunsets \\ \textit{Governed via centralized or communal tenure}} &
%                 \parbox[t]{1.5in}{\textbf{Common-Pool Resources} \\ Ocean fisheries \\ Trending topics \\ Compute clusters \\ \textit{Governed via centralized or communal tenure}} \\ \cmidrule{2-4}
%         & 
%             \multirow{4}{*}{\textit{Easy}} & 
%                 \parbox[t]{1.5in}{\textbf{Toll or Club Goods} \\ Country clubs \\ Newspaper articles \\ Paywall sites \\ \textit{Governed via private or centralized tenure}} & 
%                 \parbox[t]{1.5in}{\textbf{Private Goods} \\ Cash \\ Personal computers \\ Email addresses \\ \textit{Governed via private tenure}} \\
    
%         \bottomrule
%     \end{tabular}
%     \caption{A taxonomy of resource types, adapted from from~\cite{Hess:2007we}. A resource's type strongly determines the type of governance institution (italicized) that will manage it most effectively.}
%     \label{tab:goods_table}
% \end{table}

%\pk{Make sure we talk here about the connections to types of governance (so the table makes sense after reading the text). Cite evidence or argument for why those forms of governance are effective for those types of resources}

%The resource perspective distinguishes four types of goods (see Table~\ref{tab:goods_table}) in terms of the properties of excludability (ease of denying access to free riders) and subtractability (consumption by one prevents consumption by others). \textit{Common-pool resources} such as public server resources and user attention are non-excludable but subtractable resources.  \textit{Public goods} such as server hosting, flagging spam on a forum, posting on a social media site, or voluntarily maintaining a reputation system or other governance service are non-excludable and non-subtractable. \textit{Private goods} like currencies, account names, or personal computers are excludable and subtractable. Private goods are also called market goods because, unlike public and common pool goods, they are suitable for buying and selling through market mechanisms; markets are unable to efficiently price non-excludable goods because their use can positively or negatively affect people besides the user/owner in a way that users may not account for. \textit{Toll goods} like member-only social networks and sites with paywalls are excludable and non-subtractable. These goods have fewer collective action problems associated with them on account of their excludability. Amazon, PayPal, and eBay are all digital institutions that extend the applicability of market distribution to a greater number of participants and goods. Of course, these distinctions are not hard and fast, and it is recognized that technological and environmental factors can cause a good to change in type. For example,  ``congestible'' resources like highways and websites are public goods during low-traffic periods, but can become subtractable common pool resources as they approach the ceilings of their capacity.  

% \begin{table}[tb]
%     \small
%     \centering
%     \begin{tabular}{llp{2in}p{2in}}
        
%         & & \multicolumn{2}{c}{\textbf{Participation in governance}} \\ 
%         & & \textit{Low} & \textit{High} \\ \toprule
%         \parbox[c]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{Control granularity}}}} & 
%             \textit{Coarse} & 
%                 \textbf{Crypto \& Metrc} - unwieldy and long feedback delays; amount of resources involved in making changes, large stakeholder, highly integrated apparatus; processes are run by low accountability regulators; alternatives are forking standard or divesting; participatory during specification but \\
%                 \textbf{Subreddit editors} - moderators emerge in a bottom-up manner; within their community they are given a defined level of control.  They have no formal power to change policy or affordances at the level of Reddit policy. Resulting frictions have led to sitewide moderator strikes, themselves a coarse policy tool. &
%                 \textbf{Not possible} \\ \cmidrule{2-4}
%         & 
%             \textit{Fine} & 
%                 \textbf{Minecraft} -  & 
%                 \textbf{Wikipedia} -  \\
    
%         \bottomrule
%     \end{tabular}
%     \caption{A taxonomy of constitutional mutability along two dimensions of high or low participation and coarse or fine grained control.}
%     \label{tab:goods_table}
% \end{table}

% Definition of coarseness - do there exist agents anywhere who can implement or change the rules of the constitution
% Definition of participatory - do the participants have levers for constitutional change?

% YES/NO decision tree: instrumentation for fine-scaled constitutional change. Does there exist an agent to implement a consitutional layer?
% IF NO: Terminate, Crypto and Metrc
% If YES: next question 2
%% Q2: Can users participate in constitutional-layer change?
%% If no: Minecraft and reddit
%% If yes: Wikipedia

% Within Workshop frameworks, these categories are not objectively granted, and can change with context and circumstance.  For example, an open highway becoming congested during rush hour, or a normally low-traffic website generating viral interest both give examples of a good transitioning from public to common-pool, and the subtractability of air depends heavily on the question  (quantity of oxygen or pollutants?) and scale of inquiry (room, town, or globe?). 

%\subsection{Types of rights and roles}\label{sec:types_of_rights}
%\pk{How do the types of rights modify the types of governance we expect to be effective? \sf{\sout{There is no answer to this, but the framework allows us to answer these question.}The types of rights are really just a taxonomy that makes it possible to start asking these questions for specific systems (not even in general).  No one is going to say that these types of rights map to those types of governance always or even generally.  The spirit of this framework is really in the opposite direction of prescriptions: libertarians treat rights like a monolith, but that argument becomes less tenable when you recognize that rights are multifaceted.  The whole hope, here and in Table 1, to map constructs to prescriptions is total folly and I hope that no natural resource person reads it. So if there's a way around having to make clean prescriptions, I'm all for it.  Clean prescriptions are what Ostrom stepped in to work against. }}

%When institutions must manage resources that are not private goods, the idea of ownership as a set of rights and roles requires further decomposition. The IAD framework distinguishes between the right to \textit{access} a setting and enjoy its externalities, the right to \textit{extract} its resources, the right to \textit{participate} in the management of its resources, the right to sell or \textit{transfer} resources, and the ``meta'' right to confer or withdraw specific rights to others. 

%The specifics of a resource setting can lead to complex bundles of rights being available in different combinations to different types of stakeholders, especially when institutions include multiple types of stakeholders exercising different kinds of rights. The decomposition of rights supports a common and intuitive institutional construct: defining different types of users in terms of their differing relationships to a resource. In a canonical digital institution like Wikipedia, despite its ``free encyclopedia that anyone can edit'' mission, there are nevertheless clearly differentiated classes of ``users'' possessing distinct rights to access, share, contribute, and manage the platform across the readers, editors, and administrators.  %\brian{This example is unclear} For example, all participants in a blockchain have every kind of right, but, within a currency,  those who exercise their right to withdraw resources (to mine coins) engage preferentially in the right to manage and exchange the currency, and they also have inordinate power to exclude potential participants via the maintenance of blacklists. Miners are therefore a distinct type of user, not just in terms of their mining activity, but also from the perspective of institutional power. \pk{I agree with Brian this example was unclear. I tried to make sense of what Seth meant as best I could.}

%\subsection{Types of rules}\label{sec:types_of_rules}

%\begin{figure*}[tb]
%    \centering
%    \includegraphics[width=.75\textwidth]{images/rules.png}
%    \caption{Types of rules. Adapted from~\cite{Ostrom:2005tg}}
%    \label{fig:rules}
%\end{figure*}

%\pk{add note about ``norms'' being defined here in an unusual way. implicit vs explicit enforcement}

%Social science research on formal institutions takes a great interest in looking not just at format rules, but also how formal rules and informal norms interact to shape outcomes. 
%Despite the importance of informal norms, it is worth mentioning that informal institutions take a great interest in their formal rules, and devote great energy to ensuring that members understand and follow them.
%The IAD framework makes a distinction between \textit{rules} (which are obligatory and enforced), \textit{norms} (which are just obligatory), and \textit{strategies} (which describe suggested or possible behavior). IAD focuses most of its analytic machinery on what it calls ``rules-in-use'', which are the formal and informal statements that stakeholders use to constrain individual and  collective behavior. Rules-in-use can be one of several types, each corresponding to one of the elements of an institution.  

%According to IAD, an institution can be decomposed into a system of interacting action situations. Different types of rules can have different types of effects on the functioning of an institution. An action situation generalizes the game of economic game theory to define \emph{participants} in \emph{positions} who must decide among diverse \emph{actions} in light of the \emph{information} they possess about how actions are \emph{linked} to potential \emph{outcomes}, and the \emph{costs} and \emph{benefits} of those outcomes \cite{Ostrom:2010wk}. 

%For each of these components there is a corresponding type of rule for specifying and shaping it. \textit{Boundary rules} like server blacklists and membership applications define the actors in a system. \textit{Choice rules}, like those tacit in interface design, define the space of possible actions in the system. \textit{Position rules} define the mapping between participant types and actions, \textit{e.g.} the permissions system in Wikipedia, in which especially trusted users are permitted to perform a greater number of behaviors. Just as choice rules constrain a set of possible behaviors, \textit{scope rules} constrain the set of possible outcomes of a behavior.  \textit{Aggregation rules} map the combined actions of several actors to the possible outcomes (can everyone participate in a vote?), and \textit{payoff rules} further shape the space of possible outcomes by defining the rewards and penalties to different agents for the occurrence different outcomes.  Finally, \textit{information rules} define who will have access to what information about the system at each of its states. Figure~\ref{fig:rules} illustrates the relationship among these rules. Examples of how these different types of rules manifest in digital institutions are given in our case studies.
%Kraut and Resnick's \textit{Building Successful Online Communities}---which collect many small interventions made to different parts of different online systems---are especially rewarding to examine from the view of rules taxonomies.
